Localization-Aware Active Learning for Object Detection

Active learning - a class of algorithms that iteratively searches for the most informative samples to include in a training dataset - has been shown to be effective at annotating data for image classification. However, the use of active learning for object detection is still largely unexplored as determining informativeness of an object-location hypothesis is more difficult. In this paper, we address this issue and present two metrics for measuring the informativeness of an object hypothesis, which allow us to leverage active learning to reduce the amount of annotated data needed to achieve a target object detection performance. Our first metric measures 'localization tightness' of an object hypothesis, which is based on the overlapping ratio between the region proposal and the final prediction. Our second metric measures 'localization stability' of an object hypothesis, which is based on the variation of predicted object locations when input images are corrupted by noise. Our experimental results show that by augmenting a conventional active-learning algorithm designed for classification with the proposed metrics, the amount of labeled training data required can be reduced up to 25%. Moreover, on PASCAL 2007 and 2012 datasets our localization-stability method has an average relative improvement of 96.5% and 81.9% over the baseline method using classification only.

==> subsec_3in1.tex <==
\subsection{Combining All Cues}
\label{sec:3in1}
In order to see that if the localization uncertainty measurements have complementary information, we can further combine all cues for selecting informative images. As images with high classification uncertainty, low localization stability, and low localization tightness should be selected for annotation, the score of the $i$-th image ($I_i$) image is defined as follows:
\begin{equation}
Unc(I_i) - \lambda_{ls} Sta(I_i) - \lambda_{lt} Ti(I_i)
\end{equation} 
where $\lambda_{ls}$ and $\lambda_{lt}$ are set to 1 across all the experiments in this paper.

==> subsec_discussion_design_LT.tex <==


% \paragraph{Design of LT/C metric:}

% \textbf{*** We need better explanation for the metrics but for now I just comment it out. ***}

%% TEST-DEL-BEGIN
%
%\begin{figure}[t]
%\begin{center}
%   	\includegraphics[width=0.32\linewidth]{figures/LT_003000.jpg}
%	\includegraphics[width=0.32\linewidth]{figures/LT_006430.jpg}
%	\includegraphics[width=0.32\linewidth]{figures/LT_009039.jpg}
%	\\
%   	\includegraphics[width=0.32\linewidth]{figures/C_000622.jpg}
%	\includegraphics[width=0.32\linewidth]{figures/C_001175.jpg}
%	\includegraphics[width=0.32\linewidth]{figures/C_007048.jpg}	
%\end{center}
%   \caption{\textbf{First row:} Example images selected for annotation by method using information from localization only to evaluate the score of each box. \textbf{Second row:} Example images selected for annotation by method using classification uncertainty only (C).}
%\label{fig:LT_and_C}
%\end{figure}
%Given the measurement of localization tightness, we need to design a metric to utilize it for active learning.
%The most intuitive way is to use the localization tightness alone to decide the score for each box.
%However, in our preliminary experiments it does not help for selecting samples to annotate.
%We further analyze it by showing the images selected by different methods as shown in Fig.~\ref{fig:LT_and_C}.
%When using only localization tightness as the cue for active learning, it tends to find images (Fig.~\ref{fig:LT_and_C}, first row) that have tiny objects (e.g., airplane, bird), which are not chosen that often by other methods  (Fig.~\ref{fig:LT_and_C}, second row).
%However, these classes are easier ones that the detector already does well so that the performance of using localization tightness alone is worse than other metrics.
%More details of the experiment on different metrics using localization tightness are shown in the supplemental materials.
%
%% TEST-DEL-END 
